BLISlab: A Sandbox for Optimizing GEMM

Matrix-matrix multiplication is a fundamental operation of great importance to scientific computing and, increasingly, machine learning. It is a simple enough concept to be introduced in a typical high school algebra course yet in practice important enough that its implementation on computers continues to be an active research topic. This note describes a set of exercises that use this operation to illustrate how high performance can be attained on modern CPUs with hierarchical memories (multiple caches). It does so by building on the insights that underly the BLAS-like Library Instantiation Software (BLIS) framework by exposing a simplified "sandbox" that mimics the implementation in BLIS. As such, it also becomes a vehicle for the "crowd sourcing" of the optimization of BLIS. We call this set of exercises BLISlab.

==> DirectoryTree.tex <==
\begin{figure}[tb!]
\begin{center}
%\small
\begin{minipage}{\textwidth}
\dirtree{%
.1 Users.
.2 rvdg.
.3 blislab \DTcomment{
		\rm \color{red}
		The main directory{.} 
	}.
.4 docs \DTcomment{
			\rm \color{red}
			The directory where this document and its \LaTeX\ source exist{.} 
	}. 
.4 src \DTcomment{
			\rm \color{red}
			Directory where the source for the programming exercises exists{.} 
		}.  
.5 step1 \DTcomment{
		\rm \color{red}
		Source for step one and two of the exercise{.} 
	}.  
.5 step3 \DTcomment{
		\rm \color{red}
		Source for step three of the exercise{.} 
	}.  
.5 step\_final \DTcomment{
		\rm \color{red}
		Source for final step of the exercise{.} 
	}.  
}
\end{minipage}
\end{center}
\caption{Directory structure for the materials.  In this
example, I placed {\tt BLISF1.zip} in the home directory {\tt
  Users/rvdg} before unzipping. You may want to place it on your account's ``Desktop'' instead.}
\label{fig:dir1}
\end{figure}



==> body.tex <==



==> steps.tex <==
%\section{Step-by-step approach to the peak performance}
%Architecture: Ivy Bridge and Haswell.
%
%\subsection{Naive Approach: Three loops}
%
%\subsection{Cache Blocking: 6 loops}
%refer to GOTO paper: How to permuate to get the best loop order
%var2, var1, var3
%
%Performance Graph
%
%\subsection{Add Packing}
%
%\subsection{Micro-kernel Tricks}
%1. Butterfly or Broadcasting?
%2. Double buffering
%
%\subsection{Parameter Tuning}
%
%\subsection{Parallelization}


\begin{figure}[!htp]
  \centering
  \includegraphics[scale=.5]{figures/step1_single_thread_ivy.eps}
  \caption{Step1 performance (triple loops)}
  \label{fig:naive}
\end{figure} 

\begin{figure}[!htp]
  \centering
  \includegraphics[scale=.5]{figures/step3_single_thread_ivy.eps}
  \caption{Step3 performance (6 loops with blocking)}
  \label{fig:packing}
\end{figure} 

\begin{figure}[!htp]
  \centering
  \includegraphics[scale=.5]{figures/step10_single_thread_ivy.eps}
  \caption{Step10 performance (blocking+Intrinsics)}
  \label{fig:int}
\end{figure} 

\begin{figure}[!htp]
  \centering
  \includegraphics[scale=.5]{figures/step_final_single_thread_ivy.eps}
  \caption{Step Final performance (blocking+AVX assembly)}
  \label{fig:final}
\end{figure} 

\begin{figure}[!htp]
  \centering
  \includegraphics[scale=.5]{figures/step_final_multi_thread_ivy.eps}
  \caption{Step Final performance (multi-thread), sawtooth due to workload imbalance
in OMP threads}
  \label{fig:final_mt}
\end{figure} 





